Fast and Scalable Dialogue State Tracking with Explicit Modular Decomposition

We present a fast and scalable architecture called Explicit Modular Decomposition (EMD), in which we incorporate both classification-based and extraction-based methods and design four modules (for classification and sequence labelling) to jointly extract dialogue states. Experimental results based on the MultiWoz 2.0 dataset validates the superiority of our proposed model in terms of both complexity and scalability when compared to the state-of-the-art methods, especially in the scenario of multi-domain dialogues entangled with many turns of utterances.

==> images/data.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=0.45\textwidth]{images/data.png}
  \vspace{-0.4cm}
  \caption{Distribution of slot values in the training data. In particular, as for numbers in the legend, e.g. 100--1000 (193),``100--1000'' represents the range of the number of occurrence and ``(193)'' in the bracket denotes the number of distinct slot values. \label{fig:data}}
\end{figure}
